Massively Parallel Dynamic Programming on Trees

Dynamic programming is a powerful technique that is, unfortunately, often inherently sequential. That is, there exists no unified method to parallelize algorithms that use dynamic programming. In this paper, we attempt to address this issue in the Massively Parallel Computations (MPC) model which is a popular abstraction of MapReduce-like paradigms. Our main result is an algorithmic framework to adapt a large family of dynamic programs defined over trees. We introduce two classes of graph problems that admit dynamic programming solutions on trees. We refer to them as "(polylog)-expressible" and "linear-expressible" problems. We show that both classes can be parallelized in $O(\log n)$ rounds using a sublinear number of machines and a sublinear memory per machine. To achieve this result, we introduce a series of techniques that can be plugged together. To illustrate the generality of our framework, we implement in $O(\log n)$ rounds of MPC, the dynamic programming solution of graph problems such as minimum bisection, $k$-spanning tree, maximum independent set, longest path, etc., when the input graph is a tree.

==> general.tex <==
\subsection{Minimum Spanning Tree on Sparse Graphs}

Finding the minimum spanning tree is a fundamental problem. In fact, it is one of the main problems that Karloff et al. \cite{karloff2010model} focus on, when introducing the initial theoretical model of MapReduce. In particular, they give a constant round algorithm to find the MST of dense graphs. Moreover finding MST in metric spaces has been widely studied by \cite{yaroslavtsev2017massively, andoni2014parallel}. The total memory that they use is linear to the input size, however they give approximation algorithms for finding MST in limited metric spaces with limited dimensions. As it was noted before, obtaining constant round algorithms for general graphs is very unlikely. 

In this section, we show how our framework could be used in designing  algorithms for finding MST in general graphs. We first give an algorithm for finding exact MST in metric spaces, with arbitrary number of dimensions. 
We also give an \Ot{\log^2 n} round MST algorithm for sparse graphs. We would like to note that, there already exist efficient PRAM algorithms for minimum spanning tree problem \cite{king1997optimal} in sparse graphs. Coupling them with the simulation methods of \cite{karloff2010model, goodrich2011sorting} one can obtain distributed algorithms with almost the same round complexity. However, our main purpose in this section, is to show how our framework could be applied to sparse graphs.

%For instance we show how to use the framework that we introduced to design a \Ot{\log^2 n} round algorithm for minimum spanning tree problem of general graphs. We would like to note that, there already exist efficient parallel algorithms for minimum spanning tree problem \cite{}. Coupling them with the simulation methods of \cite{karloff2010model, goodrich2011sorting} one can obtain distributed algorithms with almost the same round complexity. The sole purpose of this section, however, is to illustrate how to go beyond trees.
\begin{theorem}\label{theorem:MST}
	Let $V$ denote a set of vectors in $d$ dimensional space and let $f$ denote a function that determines the distance between any two vectors $u$ and $v$ where $f(u,v)$ is computable in $O(d)$ space. Given any $\M$ where $\M \leq n^{2/3}$, there exists an algorithm to find MST of $V$ in \O{\log n} rounds of \model{} using $\M$ machines, such that with high probability, each machine uses a space of size at most \Ot{d \times n^{4/3}/m}.
\end{theorem}

\begin{proof}
	Let $G$ denote the metric graph of vector set $V$. any vector in $V$ represents a vertex in $G$, and the weight of an edge between any two vertex $u$ and $v$ is $f(u, v)$.
	We  partition the vertices  into $\sqrt{\M}$	 partitions, each of which containing $n / \sqrt{\M}$ vertices. Let $p_1, \dots, p_{\sqrt{\M}}$ denote the partitions. For any $i$ and $j$, where $1 \leq i < j \leq \sqrt{\M}$, we put all the vertices in $p_i$ and $p_j$ in one machine. Note that each partition is in exactly $\sqrt{\M}-1$ machines. Let $M_{i,j}$ denote the machine that contains $p_i$ and $p_j$. In this machine we find the MST between vertices in $p_i \cup p_j$, and we denote it by $T_{i,j}$. By Lemma \ref{lem:localMST} any edge $e$ that is in MST of $G$ is also in the MST between the vertices of at least one of the machines. The size of the complete graph between the vertices in one machine is $\O{(n^{4/3}/m)^2}$ so it does not fit in a single machine. To overcome this, in each machine we generate edges sequentially. We update the MST after generating any edge, and remove any edge that is not in the MST. 
	
	In the first round, the algorithm in any machine $M_{i,j}$ is as follows:  at the beginning $T_{i,j}$ is empty. For any pair of vertices $u$ and $v$ in $p_i \cup p_j$, we compute $f(u , v)$ in $O(d)$ space which is the wight of the edge $e_{i,j}$. We then add $e_{u,v}$ to $T_{i,j}$. If there was a loop in $T_{i,j}$ after adding this edge, we update $T_{i,j}$ by removing the edge with the maximum weight in this loop. Then we remove any edge that is not in $T_{i,j}$. To run this algorithm in one machine we do not need space more than \O{d \times n^{4/3}/m}, since we just store the edges of the MST. The size of the MST in each machine is at most equal to the size of the vertices in that machine which is \O{d \times n^{4/3}/m}.
	
	After the first round of the algorithm there are \O{n^{4/3}/m} edges in each machine, which is \O{n^{4/3}} in total. So, the problem of finding the MST of $G$ is now reduced to finding an MST in a graph that has $n$ vertices and \O{n^{4/3}} edges. Since there exists an algorithm that finds the MST of such a graph in $\Ot{\log{n^{4/3}}} = \Ot{\log{n}}$ rounds using $m$ machines and \Ot{n^{4/3}/m} space per machine, the number of rounds that we need to find the MST of $G$ is  \Ot{\log{n}} as well. 
	
%	To sum up, in the first round we decrease the number of edges to $\O{n^{4/3}}$ from all the possible edges of the metric graph, which is $\O{n^2}$. Then, we use an algorithm that finds the MST of the remaining edges in \Ot{\log{n}} rounds. Throughout this algorithm we use $m$ machines, and the memory per each machine is \Ot{d \times n^{4/3}/m}.
	\end{proof}

\begin{lemma} \cite{bateni2017affinity} \label{lem:localMST}
Let $M$ denote the MST of $H(V', E')$ which is a subgraph of graph $G=(V, E)$. If $e\in E'$ and $e\notin M$, then $e$ is not in the MST of $G$.
\end{lemma}

Next, we give give an \Ot{\log^2 n} round MST algorithm for sparse graphs to show how our algorithm works on sparse graphs.

\begin{theorem}
	For any given $\M$, there exists an algorithm to find the minimum spanning tree of a given graph in \Ot{\log^2 n} rounds of \model{} using $\M$ machines, such that with high probability each machine uses a space of size \Ot{n/\M} and runs an algorithm that is linear in its input size.
\end{theorem}

\newcommand{\boruvka}[0]{Bor\r uvka}

\begin{proof}[Proof sketch]
	We first explain the \boruvka{}'s famous MST algorithm, then show how to implement it as a distributed algorithm using our framework. \boruvka{}'s algorithm initially starts with $n$ \emph{components}, where each component contains one of the vertices of the graph. Defining the \emph{distance} between two components to be the minimum edge between them, \boruvka{}'s algorithm  in each step merges each component to its closest component simultaneously. It could be shown that the size of smallest component is doubled in each step, hence roughly after \O{\log n} rounds, all components are merged. The edges through which we merge these components will be the MST of the input graph.
	
	We call each round of \boruvka{} a super-round. Then show how each of the super-rounds could be implemented in \O{\log n} rounds of \model{}. Combining them together, we achieve a \Ot{\log^2 n} round algorithm for MST.
	
	Let us focus on a super round. Consider a graph that maps each component to a vertex and contains a directed edge from vertex $v$ to $u$ if the corresponding component of vertex $u$ is the closest component to the corresponding component of $v$. Assuming that no two edges of the initial graph have the same weight (which could be achieved by simply perturbing all the edge weights), the structure of this graph would be as follows. Each vertex has exactly one outgoing edge and the maximum length of a directed cycle is 2. To see this, note that if there is a cycle of size more than 2, there has to be at least two edges with the same weight. A cycle of length two indicates two components that are each other's nearest neighbors. By contracting cycles of length two, we obtain a collection of trees. In fact, each cycle of length two becomes the root of a tree. At the end of the super-round, the \boruvka{}'s algorithm merges all the components that belong to the same tree together.
	
	The idea is to use our framework to efficiently merge these trees. While merging the trees, we also have to update the distances between the contracted trees for the next super round. To do this, in the first step we make sure that all the vertices that belong to the same tree \emph{know} each other by assigning the same \emph{color} (e.g., the id of the root) to them. Note that the diameter of these trees might be arbitrarily large. Hence we need to incorporate our framework to handle this in \O{\log n} rounds. After all the vertices are assigned the color of the tree that they belong to, we find for each tree its minimum edge to other trees. Assume there are $k$ different trees. Using a $(\poly\log)$-expressible bottom-up dynamic program, for each node of a tree, we keep a list of $k-1$ different edges, where each one denotes the minimum weight edge to another tree. After this list is completely merged, we can contract the trees and remove the edges that are no longer required.
	
	Each super step takes \O{\log n} rounds. Hence the total running time of the algorithm is \Ot{\log^2 n}.
\end{proof}

\subsection{Further Applications of the Splitting Technique}
Assume that a set $V$ of vectors in a $d$-dimensional space is given in the input and a distance function $f: V \times V \to \mathbb{R}_+$ determines the distances between the input vectors. In the closest points problem, our goal is to find the pair of vectors that are closest to each other. Moreover, in the MST in metric spaces, our goal is to find the minimum-weight tree that connects all these vectors. Our goal is to come up with exact (i.e., not approximate) solutions for these problems.

Before explaining the actual algorithm, we need to mention that in the literature, with certain assumptions on the distance function or the dimension, efficient \model{} algorithms are known for finding the MST in metric spaces \cite{andoni2014parallel,  yaroslavtsev2017massively}. However, our goal here is to design a general algorithm without any assumption on the dimension or the distance function. There are two ways to consider general distance functions: (1) the value of $f$ for any two vectors is specified in the input; (2) each machine has access to an oracle that can compute the distance between any two given vectors. The former case increases the input size quadratically which simplifies the solution. For instance, finding MST in metric spaces becomes the same as finding the MST in dense (or in this case, complete) graphs for which efficient constant round \model{} algorithms are known \cite{karloff2010model, DBLP:conf/spaa/LattanziMSV11, bateni2017affinity}. Our focus, therefore, is on the latter case.

The difficulty with the oracle-based model is that the input size is of size $d \cdot |V|$ and thus we cannot fit all the vectors in one machine if we want the memory to be sublinear in the input size. On the other hand, all possible pairs of vectors have to be in the same machine at some point during the algorithm, or otherwise, we would not be able to determine the distance between them.

Let $n := d \cdot |V|$ denote the input size. To focus on the general idea, assume at first, that the number of machines $m$, is $\lceil n^{2/3} \rceil$ (instead of being given in the input) and that each machine has space $s = \Ot{n^{2/3}}$. We first randomly {\em partition} the vectors into $k = \lceil n^{1/3} \rceil$ groups $\{V_1, V_2, \ldots, V_k\}$. As an application of Chernoff bound,  the size of groups is bounded by $\Ot{n^{2/3}}$ with high probability. In the next step, for any $i \in [k]$ and $j \in [k]$ we put $V_i$ and $V_j$ in one machine. Note that the number of machines, $m = \lceil n^{2/3} \rceil$, is more than $\binom{k}{2}$ and thus we have enough machines to put each group pair in one machine.

To solve the closest points problem, in the second round (after distributing the group pairs into machines) each machine computes the minimum distance between the points that are stored in it and all machines send this minimum distance to a single machine $\mu$, then in the third round, machine $\mu$ reports the overall minimum distance. Let us denote by $S := s \cdot \M$ the overall space on all machines. For the mentioned algorithm, $S$ is $n^{4/3}$. Also, by setting $k = \sqrt{\M}$, we can get the same guarantee on $S$ as long as $\M \leq n^{2/3}$. This way, the space of each machine would be of size \Ot{n/\sqrt{m}} and therefore the overall space that the algorithm uses would be of size \Ot{n\sqrt{m}} = \Ot{n^{4/3}}.

\begin{remark}
	For any given $\M$ where $\M \leq n^{2/3}$, there exists an algorithm to solve the oracle-based closest points problem in 3 rounds of \model{} using $\M$ machines, such that with high probability, each machine uses a space of size at most \Ot{n^{4/3}/m}.
\end{remark}

But can we get any better bounds on $S$? Obviously if there are very few machines with large memories we can improve this bound. However, the goal in distributed settings is to parallelize the work-load into as many machines as possible. More precisely, for a given overall space $S$, we want to able to have as many as $m = \lfloor \sqrt{S} \rfloor$ machines, each with memory $s \leq S/m = \O{\sqrt{S}}$. (Recall that in \model{} we assume $m \leq s$, therefore $m^2 \leq s \cdot m = S$ and thus $m \leq \sqrt{S}$. Meaning that $m = \lfloor \sqrt{S} \rfloor$ is the maximum number of machines one can hope for.) With this natural assumption, we get the following result implying that the $n^{4/3}$ overall space is in some sense tight.

\begin{lemma}
	If $m = \lfloor \sqrt{S} \rfloor$, any algorithm in \model{} that solves the oracle-based closest points problem requires at least $\Omega(n^{4/3})$ overall space.
\end{lemma}

We defer the proof of the following theorem about finding MST in metric spaces to the forthcoming sections. However, using the ``splitting'' idea, we can first {\em sparsify} the complete distance graph such that we can randomly distribute its edges in the machines and then solve the MST problem on a sparse graph.\\
\\
\textbf{Theorem \ref{theorem:MST}.} (restated)	
		Let $V$ denote a set of vectors in $d$ dimensional space and let $f$ denote a function that determines the distance between any two vectors $u$ and $v$ where $f(u,v)$ is computable in $O(d)$ space. Given any $\M$ where $\M \leq n^{2/3}$, there exists an algorithm to find MST of $V$ in \O{\log n} rounds of \model{} using $\M$ machines, such that with high probability, each machine uses a space of size at most \Ot{d \cdot n^{4/3}/m}.




==> general_notes.tex <==
\clearpage

\section{Notes - To be deleted}
\mdcomment{Very important: do not forget to define $m=n^\delta$  }
\sbcomment{Somewhere denote the set of available machines by \Mset{}}

\sbcomment{For simplicity of calculations, we also assume $\M = 2^k$ for some integer $k$ \footnote{This assumption does not restrict the model since for any integer $\M$, there exists an integer $k$ such that $\frac{\M}{2} \leq 2^k \leq \M$. Therefore, even if $\M$ is not a power of 2, one can assume that the algorithm uses only $2^k$ of the available machines. This does not asymptotically change the available space either since $2^k = \O{\M}$.}. }

\sbcomment{Don't forget to check if everything in the list is mentioned in the intro.}

\sbcomment{Explain somewhere that random decompositions don't work}

To be defined:
\begin{enumerate}
	\item Define $V(G)$, $E(G)$ for a graph.
	\item $[n]=\{1, \dots, n\}$ and $[i, j] = \{i, i+1, \dots, j\}$ (this is probably a bad notation, confused with ranges)
\end{enumerate}


\paragraph{Introduction.} 
\begin{enumerate}
	\item Model:
	\begin{enumerate}
		\item Motivation behind the model (\cite{im2017efficient} is a good source)
		\item Other papers on the same model. Most important ones are probably \cite{andoni2014parallel} and \cite{im2017efficient}.
		\item How the model relates to previous parallel models, e.g., PRAM. (\cite{andoni2014parallel} argues we can achieve faster algorithms in this model compared to PRAM)
	\end{enumerate}
	\item Motivation.
	\begin{enumerate}
		\item Comparison to other graph algorithms (they usually have access to all nodes in any machine).
		\item We give the first sublinear algorithm for graphs in parallel setting.
		\item ``Is there a black box that given a sequential dynamic programming for a problem defined on trees, converts it to a parallel algorithm?"
	\end{enumerate}
	\item Previous work.
	\begin{enumerate}
		\item We have not been able to find any sub-linear parallel algorithms for graph problems. Maybe we should consider a broader scope?
	\end{enumerate}
	\item Our contributions. \sbcomment{This part has to be written after the technical part is complete. I will write it.}
	\item Generalizations to graphs. \sbcomment{This will have its own section. Still not completely sure about what will be there. Things that we will probably explain in that section: random spanning trees. (they are useful in practice. Assigning weights, etc.) FRT/Racke for approximations.}
	%		\begin{enumere}
\end{enumerate}

==> kcenter.tex <==

In this section we present two linear-expressible, 
splittable dynamic programs for
\kcenter\ and \kmedian\ on trees, which coupled with
Theorem~\ref{thm:linear-expressible} yield sublinear-space distributed
algorithms.

\subsection{\kmedian\ on trees}
We begin with restating a dynamic program (DP) from~\cite{Shah:DP} for
\kmedian\ on trees.  A similar DP was originally given 
by~\cite{Tamir:DP}, but we use the reformulation 
in~\cite{Shah:DP}, which provides slightly better bounds that are
necessary to prove the properties of Theorem~\ref{thm:linear-expressible}.   
This DP requires $O(kn_v)$ space at
a tree node $v$ with $n_v$ descendants, 
and spends $O(k^2n_v)$ time to compute all entries at
node $v$ from the solutions corresponding to its children.

Let $T(V, E)$ be a tree rooted at $r\in V$.  We denote by $T_v$ the
subtree rooted at $v\in V$.  Let $G_v^p(x)$ for $v\in V$, $0\leq p\leq
k$ and $x\geq 0$, be the minimum value of the \kmedian\ objective for
the subproblem defined on $T_v$ that uses only $p$ medians, at least one
of which is guaranteed to be within distance $x$ of $v$.  Similarly let
$F_v^p(x)$ for $v\in V$, $0\leq p\leq k$ and $x\geq 0$, be the minimum
value of the \kmedian\ objective for the subproblem defined on $T_v$
that uses only $p$ medians if a median within distance $x$ of $v$
(outside $T_v$) is guaranteed to have been selected.

The solution we seek is $F^k_r(\infty) = G^k_r(\infty)$.  Although the
functions $F_v^p(x)$ and $G_v^p(x)$ are defined over a continuous range 
for $x$, these are piecewise linear functions with $O(n_v)$ 
breakpoints~\cite{Shah:DP}.  There
is no need to know these breakpoints initially, as all the operations
can be performed on a concise representation consisting of $(x, y)$
pairs where $y$ is the value of the function at $x$.
Shah~\cite{Shah:DP} shows how a binary search can be used to obtain
the function value for any continuous $x$, since the two functions $G$
and $F$ are monotone in $x$ (decreasing and increasing, respetively).

If $v$ is a leaf in the tree,
\begin{align}
 G_v^0(x) &= \infty, & F_v^0(x) &= x, & \text{and} \\
 G_v^p(x) &= 0, & F_v^p(x) &= 0, & \text{for $p > 0$}.
\end{align}

For a non-leaf node $v$ with children $a$ and $b$, let $x_a$ and $x_b$
denote the distance of $v$ to $a$ and $b$, respectively.  
We have
\begin{align}
 F_v^p(x) &= \min [ G_v^p(\infty), \min_{0\leq i\leq p} \{x+F_a^i(x+x_a)+F_b^{p-i}(x+x_b)\}], \\
 G_v^p(0) &= \min_{0\leq i\leq p-1} \{F_a^i(x_a)+F_b^{p-1-i}(x_b)\}.  \label{eqn:kmedian:4}
\end{align}
Now let $x_1 \leq x_2 \leq \dots$ denote the distances of $v$ to all
its descendants.  For children $a$ and $b$, we use the
notation $T_a$ and $T_b$ to refer the subtrees rooted at each child,
respectively.  If $x_m$ corresponds to the distance of $v$ to a node
in $T_a$, we get
\begin{align}
 G_v^p(x_m) &= \min [ G_v^p(x_{m-1}), \min_{0\leq i\leq p} \{x_m+G_a^i(x_m-x_a)+F_b^{p-i}(x_m+x_b)\}], 
\intertext{and for the case of $x_m$ corresponding to the distance of $v$ to a node in $T_b$,}
 G_v^p(x_m) &= \min [ G_v^p(x_{m-1}), \min_{0\leq i\leq p} \{x_m+G_b^i(x_m-x_b)+F_a^{p-i}(x_m+x_a)\}].
\end{align}

Clearly we have a vector of length $O(kn_v)$ at each node of the tree.
To compute each entry, we need to look at $O(k)$ entries from the
children, hence a total runtime of $O(k^2n)$, as claimed.

Combining this dynamic program with
Theorem~\ref{thm:linear-expressible}, we obtain, for $k = \poly\log n$,
a distributed algorithm for \kmedian\ on trees, that runs
in $\tilde O(\log n)$ rounds of \model\ using $m$ machines, such that
with high probability each machine uses $\tilde O(n^{1+\epsilon}/m)$
space and $\tilde O(n^2/m)$ time per round.

This argument requires us to prove certain properties about the above DP.
Here we provide the sketch of the proof.
The DP is binary adaptable, because we can accommodate ``auxiliary''
nodes in the computation.  By construction leaves are not auxiliary.
Among the recursive equations, only \eqref{eqn:kmedian:4} provisions
a median at $v$, which should be changed to $G_v^p(0) = \infty$
if $v$ is an auxiliary.
When $k = \poly\log n$, the total size of the DP table at node $v$
is $O(kn_v) = \tilde O(n_v)$.
%
To establish splittability, we partition the piecewise linear function
into $m$ continuous pieces of almost the same size.
We try the cross product of these divisions and whenever we get a
possibility (i.e., one of the terms in the minimization) for either
$G_v^p(x)$ or $F_v^p(x)$, we send the result to the corresponding
machine.  Note that each recursive formula takes the minimum among
$O(k)$ possibilities, hence the resulting coming in can be easily
aggregated.


\subsection{\kcenter\ on trees}
Next we demonstrate how the above dynamic program can be adapted to solve
\kcenter, providing similar bounds for space usage and running time.
Afterwards we explain how to improve the bounds, such that the results
extends to arbitrary values of $k$.

We define the functions $F_v^p(x)$ and $G_v^p(x)$ exactly as above,
however, the objective value is now the maximum distance of a node
within the subproblem to its closest center (rather than sum of these
distances).

Here we only rewrite the adapted formulas for \kcenter\ DP,
where most of the additions have changed to maximizations.
The proof of correctness is similar to that in~\cite{Shah:DP},
and is deferred to the full version of the paper.

If $v$ is a leaf in the tree, the formulas are exactly as those
for \kmedian:
\begin{align}
 G_v^0(x) &= \infty, & F_v^0(x) &= x, & \text{and} \\
 G_v^p(x) &= 0, & F_v^p(x) &= 0, & \text{for $p > 0$}.
\end{align}

For a non-leaf node $v$, we have
\begin{align}
 F_v^p(x) &= \min [ G_v^p(\infty), \min_{0\leq i\leq p} \max\{x,F_a^i(x+x_a),F_b^{p-i}(x+x_b)\}], \\
 G_v^p(0) &= \min_{0\leq i\leq p-1} \max\{F_a^i(x_a),F_b^{p-1-i}(x_b)\}.
\end{align}
If $x_m$ corresponds to the distance of $v$ to a node
in $T_a$, we get
\begin{align}
 G_v^p(x_m) &= \min [ G_v^p(x_{m-1}), \min_{0\leq i\leq p} \max\{x_m,G_a^i(x_m-x_a),F_b^{p-i}(x_m+x_b)\}], 
\intertext{and for the case of $x_m$ corresponding to the distance of $v$ to a node in $T_b$,}
 G_v^p(x_m) &= \min [ G_v^p(x_{m-1}), \min_{0\leq i\leq p} \max\{x_m,G_b^i(x_m-x_b),F_a^{p-i}(x_m+x_a)\}].
\end{align}



Notice that we can combine this dynamic program with 
Theorem~\ref{thm:linear-expressible}, as we did for that
of \kmedian, to obtain similar bounds on the number of rounds, running
time and space usage per round.  

%\subsection{Extensions}
%
%We expect that this idea can be extended to several other problems,
%including facility location problem, minimum diameter, $k$-partitioning, $k$-median, and $k$-center, because they have similar dynamic programming solutions
%when the input graph is a tree.
%We defer the detailed discussion to
%the full version of the paper.


==> polylog-summary.tex <==
\section{Warm-Up: Solving $(\poly\log)$-Expressible Problems}\label{sec:polylogsummary}

The first problem in solving dynamic programs on trees is that there is no guarantee on the depth of the tree. If the given tree has only logarithmic depth one can obtain a logarithmic round algorithm by simulating a bottom-up dynamic program in parallel, where nodes at the same level are handled in the same round simultaneously. Unfortunately the input tree might be quite unbalanced, with superlogarithmic depth.

To resolve this issue, we adopt a celebrated {\em tree contraction} method of parallel computing to our model. Roughly speaking, the algorithm decomposes the tree into pieces of bounded size, with small interdependence. The latter property allows us to almost independently solve the subproblems. To remain self-contained, we describe the tree decomposition algorithm and its proof in Appendix~\ref{sec:treedecomposition}. The following theorem is an informal restatement of the main result of that section.

\vspace{0.2cm}
\noindent \textbf{Theorem \ref{thm:decomposebinary}.} (Informal restatement)
	There exists a randomized algorithm that converts any given tree to a binary version of it and then decomposes the binary tree into connected subgraphs of bounded size such that each subgraph can be stored in one machine and is connected to at most 3 other subgraphs. For any given \M{}, the algorithm uses \M{} machines and with high probability terminates in $\O{\log n}$ rounds of \model{}. Each machine uses a memory of size at most $\Ot{n/\M}$ and runs an algorithm that is linear in its memory size.
\vspace{0.2cm}

To motivate the need to use an involved decomposition algorithm, we first give hints on why trivial approaches do not work. A natural (trivial) algorithm is to choose a set of randomly selected \emph{joint} edges (or vertices) and divide the tree based on them. Note that the main difficulty is that we need to bound the size of the largest component with a high probability. It could be shown that this trivial algorithm, even for the simple case of full binary trees fails. More precisely, it could be shown that the size of the component that contains the root is of size $\Omega(n)$ (instead of $\Ot{n/m}$) with a high probability.

\paragraph{Overview of Tree Decomposition.} At first,  the input tree is converted into a binary tree. To do this, the algorithm first computes the degree of each vertex and then adds the needed \emph{auxiliary} vertices to it. After that, roughly, the challenge is that the vertices have little knowledge about their status in the tree (e.g., they do not know their depth) and all the decomposition happens using the local information that is accessible to the vertices. To do this, the algorithm proceeds in \emph{phases} (not rounds). In each phase, the algorithm \emph{selects} a subset of vertices based on a set of local rules such as their degree, status of their parent, etc. Next, each vertex is \emph{merged} to its closest selected ancestor. Interestingly, it can be proved that in fact these local rules guarantee that the size of the maximum component is bounded by \Ot{n/m} with high probability.

After decomposing the tree into pieces that each can be stored in one machine, we can solve $(\poly\log)$-expressible problems as follows. We first use the compressor algorithm that is guaranteed to exist for $(\poly\log)$-expressible problems and store a data of size at most $\poly\log(n)$ bits for each component. Then in the next step, since there are at most \Ot{m} components, we can send the partial data of all components into one machine. Then in only one round, we merge all these partial data sequentially in one machine; obtaining the following result.

\xhdr{Theorem~\ref{thm:polylog-expressible}.} For any given $\M$, there exists an algorithm to solve any $(\poly\log)$-expressible problem in \O{\log n} rounds of \model{} using $\M$ machines, such that with high probability each machine uses a space of size \Ot{n/\M} and runs an algorithm that is linear in its input size.
\vspace{0.2cm}
	
We defer the formal proof of this theorem and examples of $(\poly\log)$-expressible problems to Appendix~\ref{sec:polylogexpressible}.


	

==> splittability__mahsa_derakhshan_s_conflicted_copy_2018-02-26_.tex <==
\section{Towards Solving Linear-Expressible Problems: Splitting Technique}\label{sec:splittability} 
The main goal of this section is to define a property called ``splittability'' for linear-expressible problems, that indeed holds for the aforementioned linear-expressible problems and prove, by using a total memory of \Ot{n^{4/3}}, we are able to parallelize linear-expressible problems that are splittable in \Ot{\log n} rounds. The main reason behind the need to define this extra property for linear-expressible problems, is that in contrast to $(\poly\log)$-expressible problems, the partial data of the subtrees in linear-expressible problems might have a relatively large size, hence when merging two subtrees, we are not able to access their partial data in one machine. As a result, we need to be able to distribute the merging step among different machines. It is worth mentioning that we prove the total memory of \Ot{n^{4/3}} is in some sense tight, unless we limit the number of machines to be too small, which defeats the purpose of MapReduce, which is to have maximum possible parallelization.

\newcommand{\subunifier}{\ensuremath{\mathcal{S}}}
\newcommand{\unifier}{\ensuremath{\mathcal{U}}}
\renewcommand{\vector}[1]{\ensuremath{\vec{\compressor(#1)}}}


We first describe a natural technique in {\em splitting} a problem that results in obtaining \model{} algorithms for a wide variety of problems. This technique is not specific to trees. In fact, to illustrate the key ideas, we begin by solving the closest points and minimum spanning tree problems on general metric spaces.


\subsection{Key Ideas: Closest Points and MST on Metric Spaces}
A set $V$ of vectors in a $d$-dimensional space is given in the input and a distance function $f: V \times V \to \mathbb{R}_+$ determines the distances between the input vectors. In the closest points problem, our goal is to find the pair of vectors that are closest to each other. Moreover, in the MST in metric spaces, our goal is to find the minimum-weight tree that connects all these vectors. Our goal is to come up with exact (i.e., not approximate) solutions for these problems.

Before explaining the actual algorithm, we need to mention that in the literature, with certain assumptions on the distance function or the dimension, efficient \model{} algorithms are known for finding the MST in metric spaces \cite{andoni2014parallel,  yaroslavtsev2017massively}. However, our goal here is to design a general algorithm without any assumption on the dimension or the distance function. There are two ways to consider general distance functions: (1) the value of $f$ for any two vectors is specified in the input; (2) each machine has access to an oracle that can compute the distance between any two given vectors. The former case increases the input size quadratically which simplifies the solution. For instance, finding MST in metric spaces becomes the same as finding the MST in dense (or in this case, complete) graphs for which efficient constant round \model{} algorithms are known \cite{karloff2010model, DBLP:conf/spaa/LattanziMSV11, bateni2017affinity}. Our focus, therefore, is on the latter case.

The difficulty with the oracle-based model is that the input size is of size $d \cdot |V|$ and thus we cannot fit all the vectors in one machine if we want the memory to be sublinear in the input size. On the other hand, all possible pairs of vectors have to be in the same machine at some point during the algorithm, or otherwise, we would not be able to determine the distance between them.

Let $n := d \cdot |V|$ denote the input size. To focus on the general idea, assume at first, that the number of machines $m$, is $\lceil n^{2/3} \rceil$ (instead of being given in the input) and that each machine has space $s = \Ot{n^{2/3}}$. We first randomly {\em partition} the vectors into $k = \lceil n^{1/3} \rceil$ groups $\{V_1, V_2, \ldots, V_k\}$. As an application of Chernoff bound,  the size of groups is bounded by $\Ot{n^{2/3}}$ with high probability. In the next step, for any $i \in [k]$ and $j \in [k]$ we put $V_i$ and $V_j$ in one machine. Note that the number of machines, $m = \lceil n^{2/3} \rceil$, is more than $\binom{k}{2}$ and thus we have enough machines to put each group pair in one machine.

To solve the closest points problem, in the second round (after distributing the group pairs into machines) each machine computes the minimum distance between the points that are stored in it and all machines send this minimum distance to a single machine $\mu$, then in the third round, machine $\mu$ reports the overall minimum distance. Let us denote by $S := s \cdot \M$ the overall space on all machines. For the mentioned algorithm, $S$ is $n^{4/3}$. Also, by setting $k = \sqrt{\M}$, we can get the same guarantee on $S$ as long as $\M \leq n^{2/3}$. This way, the space of each machine would be of size \Ot{n/\sqrt{m}} and therefore the overall space that the algorithm uses would be of size \Ot{n\sqrt{m}} = \Ot{n^{4/3}}.

\begin{remark}
	For any given $\M$ where $\M \leq n^{2/3}$, there exists an algorithm to solve the oracle-based closest points problem in 3 rounds of \model{} using $\M$ machines, such that with high probability, each machine uses a space of size at most \Ot{n^{4/3}/m}.
\end{remark}

But can we get any better bounds on $S$? Obviously if there are very few machines with large memories we can improve this bound. However, the goal in distributed settings is to parallelize the work-load into as many machines as possible. More precisely, for a given overall space $S$, we want to able to have as many as $m = \lfloor \sqrt{S} \rfloor$ machines, each with memory $s \leq S/m = \O{\sqrt{S}}$. (Recall that in \model{} we assume $m \leq s$, therefore $m^2 \leq s \cdot m = S$ and thus $m \leq \sqrt{S}$. Meaning that $m = \lfloor \sqrt{S} \rfloor$ is the maximum number of machines one can hope for.) With this natural assumption, we get the following result implying that the $n^{4/3}$ overall space is in some sense tight.

\begin{lemma}
	If $m = \lfloor \sqrt{S} \rfloor$, any algorithm in \model{} that solves the oracle-based closest points problem requires at least $\Omega(n^{4/3})$ overall space.
\end{lemma}

We defer the proof of the following theorem about finding MST in metric spaces to the forthcoming sections. However, using the ``splitting'' idea, we can first {\em sparsify} the complete distance graph such that we can randomly distribute its edges in the machines and then solve the MST problem on a sparse graph.\\
\\
\textbf{Theorem \ref{theorem:MST}.} (restated)	
		Let $V$ denote a set of vectors in $d$ dimensional space and let $f$ denote a function that determines the distance between any two vectors $u$ and $v$ where $f(u,v)$ is computable in $O(d)$ space. Given any $\M$ where $\M \leq n^{2/3}$, there exists an algorithm to find MST of $V$ in \Ot{\log n} rounds of \model{} using $\M$ machines, such that with high probability, each machine uses a space of size at most \Ot{d \cdot n^{4/3}/m}.


\subsection{Splittability for Linear-Expressible Problems}
The splittability property is a generalization of the techniques used for the aforementioned problems in {\em splitting} the points into groups and putting each pair of groups in one machine.

Intuitively, a problem instance $P$ is splittable if it is possible to represent it with a set of $n$ {\em objects} such that the output of the problem depends only on the pair-wise relations of these objects. In the DP context, the splittability property is useful for linear-expressible problems. Recall that the partial data of a subtree $T$ in linear-expressible problems could be linear in the size of that subtree and thus could be as large as $\Omega(n)$ and hence cannot be stored in one machine which has only sublinear space in $n$. Therefore for obtaining the partial data of a node $u$, we need to come up with distributed solutions in merging the partial data of its children. The splittability property ensures that these partial data can be effectively merged using the splitting technique.

\begin{definition}[Splittability] \label{def:Splittability}
	Consider a linear-expressible problem $P$ and a binary adapted dynamic program \sol{P} for it. We know since $P$ is a linear-expressible problem, for any subtree $T$ of \Tb{} with $n_T$ vertices, a compressor function returns a partial data of size at most \Ot{n_T} if at most a constant number of the leaves of $T$ are unknown. Denote this partial data by $\compressor(T)$. 
	We say problem $P$ is splittable, if for any given connected subtree $T'$ of \Tb{}, the partial data $\compressor(T')$ can be represented as a vector $\vector{T'}$ of at most $\Ot{n_{T'}}$ elements such that for any connected subtrees $T_1$ and $T_2$ of \Tb{} that are connected with an edge (with $T$ being $T_1 + T_2$) the following condition holds. There exist two algorithms \subunifier{} (sub unifier) and \unifier{} (unifier) such that for any consecutive partitioning $(P_1, P_2, \ldots, P_{k_1})$ of \vector{T_1} and any consecutive partitioning $(Q_1, Q_2, \ldots, Q_{k_2})$ of \vector{T_2},
	\begin{enumerate}
		\item Algorithm $\subunifier(P_i, Q_j)$ returns a vector of size at most $|P_i| + |Q_j|$ in time $\poly(|P_i|+|Q_j|)$ such that each element of this vector ``affects" at most one element of \vector{T}.
		\item Given the elements in $\subunifier(P_i, Q_j)$ that ``affect" an element $a$ in \vector{T} for every  $1 \leq i \leq k_1$ and $1 \leq j \leq k_2$, $\unifier$ computes the value of element $a$ using linear space and polynomial time in input size.
	\end{enumerate}
	\mdcomment{Mention bisection and refer to its proof. One can find examples of sub unifier and unifier functions there.}
\end{definition}

%
%Without loss of generality we assume this data is a vector of size $\Ot{n_T}$ and denote it by $\compressor(T)$.
%	
%	We say problem $P$ is splittable, if there exist two algorithms $\splitter$ (splitter) and \unifier{} (unifier) such that for any given subtree $T'$ and an integer $s$, $\splitter(\compressor(T'), s)$ splits vector $\compressor(T)$ into sub-vectors of size $s$ with the following properties. Let $T_1$ and $T_2$ be two subtrees that have a common vertex and let $T$ denote the subtree that is obtained by merging $T_1$ and $T_2$. Let $(a_1, a_2, \ldots, a_k) = \splitter(\compressor(T_1), s)$ and let $(b_1, b_2, \ldots, b_{k'}) = \splitter(\compressor(T_2), s)$.
%	\begin{enumerate}
%		\item Function $\unifier(p_1, p_2)$ returns a vector of size $2s$ where each element of it affects only one element in $\compressor(T)$.
%		\item Any element in $\compressor(T)$ could be computed based on the output of the unifier that affect it.
%	\end{enumerate}

We show with a slightly more total space (the space on each machine is still sublinear) it is possible to design parallel algorithms in \Ot{\log n} rounds for linear-expressible problems if they are splittable.

\sbcomment{Remove it --- or not.}
\begin{theorem}\label{thm:linear-expressible}
	For any given $\M$, there exists an algorithm to solve any linear-expressible problem that is splittable in \Ot{\log n} rounds of \model{} using $\M$ machines, such that with high probability each machine uses a space of size \Ot{n^{4/3}/\M}, and runs an algorithm that is polynomial in its space size for some $0 < \eps < 1$.
\end{theorem}

As a corollary of Theorem~\ref{thm:linear-expressible}, we give logarithmic round algorithms for minimum bisection, and $k$-spanning tree problems using an overall space of $\Ot{n^{1+\eps}}$ for some constant $\eps < 1$.


==> to_comment.tex <==
  
	To prove that during the algorithm, with high probability no machine violates the memory limit of $\Ot{n/\M}$, it suffices to prove that with high probability the number of vertices with degree greater than $d_{max}$ in any machine $\mu \in \Mset$ is $\Ot{1}$, since it yields that the size of the message each machine sends in round 1 of the algorithm is $ \Ot{1}$, and hence we have $\Ot{\M} \leq  \Ot{n/\M}$, the overall message passing for each machine does not violate the memory limit. Moreover, it indicates that the total number of vertices added to each machine is $\Ot{n/\M}$ since it is at most $ \Ot{1} \cdot {\frac{n}{d_{max}}} \leq \Ot{n/\M}$ for any machine  in $\Mset$. To prove this claim, we use two facts. First, before running the algorithm we uniformly distribute the vertices over all the machines, and the second is that the total number of the vertices with degree at least $d_{max}$ in a tree is at most $\O{\frac{n}{d_{max} } }\leq \O{\M}$. So, by Claim \ref{claim:balls-logwise} with high probability there are at most $\Ot{1}$  vertices with degree at least $d_{max}$ in any machine $\mu \in \Mset$.
	
		\begin{algorithm}[h]
		\caption{An algorithm to convert a given tree \T{} to a bounded degree tree $\T^d{}$, an extension of \T{}}
		\label{alg:Tree-log}
		\begin{algorithmic}[1]
			
			\Require{given a number $d_{max}$  this algorithm converts a tree \T{} whose vertices are  distributed  over $\M$ machines to an extension of it, $\T^d{}$ with maximum degree $\Ot{d_{max}}$}
			
			\State Let $\mu$ denote the machine in which this instance of algorithm is running, and let $V_\mu$ denote the set of vertices of $\T{}$  that are stored in this machine.
			\Round{1}
			\State Let $S_\mu$ be a dictionary with the set of keys $K_\mu=\{\ind{v} |\deg(v)> d_{max}, v\in V_\mu\}$.
			\State For any $v$, such that $\ind{v}\in K_\mu$, $S_\mu(\ind{v}) = \lceil\frac{\deg(v)}{d_{max}}\rceil$. \mdcomment{deg(v) ?? children(v)}
			\State Send $S_\mu$ and $K_\mu$ to all the other machines.
			\EndRound
			\Round{2}
			\State $K \leftarrow \cup_{i \in \Mset} K_i$
			\State  $S \leftarrow \cup_{i \in \Mset} S_i$ \Comment{Since $K_i$s are distinct, for any $i\in K$ S[i] has exactly one value}
			
			\State Let $D$ be a dictionary on the same set of keys as $S$, while for any  $i\in K$, $D[i]=n+\Sigma_{j\in S, j<i}S[j]$.
			\For {every $v$ in $V_\mu$}
			\If{$\parent{v} \in K $}
			\State	Choose $x$ uniformly at random from $[S(\ind{v})]$.
			\State   $\parent{v}\leftarrow D[\parent{v}]+ x$ 	\Comment{$D[\parent{v}]+ x$ is a unique index in the range $ [n, 2n]$ assigned to the $x$-th child of vertex v in $\T^d{}$}
			\EndIf
			\EndFor
			\For{every $v$ in $K_\mu$}
			\For{every $j$ in $[S[v]]$}
			\State Add Vertex$(v, D[v]+j)$ to $V_\mu$ .
			\EndFor
			\EndFor
			\EndRound
		\end{algorithmic}
	\end{algorithm}
	\end{proof}
